Domain Aggregation Networks for Multi-Source Domain Adaptation

In many real-world applications, we want to exploit multiple source datasets of similar tasks to learn a model for a different but related target dataset -- e.g., recognizing characters of a new font using a set of different fonts. While most recent research has considered ad-hoc combination rules to address this problem, we extend previous work on domain discrepancy minimization to develop a finite-sample generalization bound, and accordingly propose a theoretically justified optimization procedure. The algorithm we develop, Domain AggRegation Network (DARN), is able to effectively adjust the weight of each source domain during training to ensure relevant domains are given more importance for adaptation. We evaluate the proposed method on real-world sentiment analysis and digit recognition datasets and show that DARN can significantly outperform the state-of-the-art alternatives.

==> definitions.tex <==
\RequirePackage{latexsym}
\RequirePackage{amsmath}
% \RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{bm}

\newcommand{\defeq}{\overset{\text{\tiny def}}{=}}
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

\newcommand{\thetaset}{\Theta}
\newcommand{\normal}{\mathcal{N}}
\newcommand{\hilbertspace}{\mathcal{H}}

%%%%%%%% Stock standard definitions %%%%%%%%%%%%%%%

\newcommand{\ab}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\cbb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\lb}{\mathbf{l}}
\newcommand{\mb}{\mathbf{m}}
\newcommand{\nbb}{\mathbf{n}}
\newcommand{\ob}{\mathbf{o}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\sbb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\zb}{\mathbf{z}}

\newcommand{\abtil}{\tilde{\ab}}
\newcommand{\bbtil}{\tilde{\bb}}
\newcommand{\cbtil}{\tilde{\cbb}}
\newcommand{\dbtil}{\tilde{\db}}
\newcommand{\ebtil}{\tilde{\eb}}
\newcommand{\fbtil}{\tilde{\fb}}
\newcommand{\gbtil}{\tilde{\gb}}
\newcommand{\hbtil}{\tilde{\hb}}
\newcommand{\ibtil}{\tilde{\ib}}
\newcommand{\jbtil}{\tilde{\jb}}
\newcommand{\kbtil}{\tilde{\kb}}
\newcommand{\lbtil}{\tilde{\lb}}
\newcommand{\mbtil}{\tilde{\mb}}
\newcommand{\nbtil}{\tilde{\nbb}}
\newcommand{\obtil}{\tilde{\ob}}
\newcommand{\pbtil}{\tilde{\pb}}
\newcommand{\qbtil}{\tilde{\qb}}
\newcommand{\rbtil}{\tilde{\rb}}
\newcommand{\sbtil}{\tilde{\sbb}}
\newcommand{\tbtil}{\tilde{\tb}}
\newcommand{\ubtil}{\tilde{\ub}}
\newcommand{\vbtil}{\tilde{\vb}}
\newcommand{\wbtil}{\tilde{\wb}}
\newcommand{\xbtil}{\tilde{\xb}}
\newcommand{\ybtil}{\tilde{\yb}}
\newcommand{\zbtil}{\tilde{\zb}}

\newcommand{\atil}{\tilde{a}}
\newcommand{\btil}{\tilde{b}}
\newcommand{\ctil}{\tilde{c}}
\newcommand{\dtil}{\tilde{d}}
\newcommand{\etil}{\tilde{e}}
\newcommand{\ftil}{\tilde{f}}
\newcommand{\gtil}{\tilde{g}}
\newcommand{\htil}{\tilde{h}}
\newcommand{\itil}{\tilde{i}}
\newcommand{\jtil}{\tilde{j}}
\newcommand{\ktil}{\tilde{k}}
\newcommand{\ltil}{\tilde{l}}
\newcommand{\mtil}{\tilde{m}}
\newcommand{\ntil}{\tilde{n}}
\newcommand{\otil}{\tilde{o}}
\newcommand{\ptil}{\tilde{p}}
\newcommand{\qtil}{\tilde{q}}
\newcommand{\rtil}{\tilde{r}}
\newcommand{\stil}{\tilde{s}}
\newcommand{\ttil}{\tilde{t}}
\newcommand{\util}{\tilde{u}}
\newcommand{\vtil}{\tilde{v}}
\newcommand{\wtil}{\tilde{w}}
\newcommand{\xtil}{\tilde{x}}
\newcommand{\ytil}{\tilde{y}}
\newcommand{\ztil}{\tilde{z}}

\newcommand{\ahat}{\hat{a}}
\newcommand{\bhat}{\hat{b}}
\newcommand{\chat}{\hat{c}}
\newcommand{\dhat}{\hat{d}}
\newcommand{\ehat}{\hat{e}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\ghat}{\hat{g}}
\newcommand{\hhat}{\hat{h}}
\newcommand{\ihat}{\hat{i}}
\newcommand{\jhat}{\hat{j}}
\newcommand{\khat}{\hat{k}}
\newcommand{\lhat}{\hat{l}}
\newcommand{\mhat}{\hat{m}}
\newcommand{\nhat}{\hat{n}}
\newcommand{\ohat}{\hat{o}}
\newcommand{\phat}{\hat{p}}
\newcommand{\qhat}{\hat{q}}
\newcommand{\rhat}{\hat{r}}
\newcommand{\shat}{\hat{s}}
\newcommand{\that}{\hat{t}}
\newcommand{\uhat}{\hat{u}}
\newcommand{\vhat}{\hat{v}}
\newcommand{\what}{\hat{w}}
\newcommand{\xhat}{\hat{x}}
\newcommand{\yhat}{\hat{y}}
\newcommand{\zhat}{\hat{z}}

\newcommand{\abhat}{\hat{\ab}}
\newcommand{\bbhat}{\hat{\bb}}
\newcommand{\cbhat}{\hat{\cb}}
\newcommand{\dbhat}{\hat{\db}}
\newcommand{\ebhat}{\hat{\eb}}
\newcommand{\fbhat}{\hat{\fb}}
\newcommand{\gbhat}{\hat{\gb}}
\newcommand{\hbhat}{\hat{\hb}}
\newcommand{\ibhat}{\hat{\ib}}
\newcommand{\jbhat}{\hat{\jb}}
\newcommand{\kbhat}{\hat{\kb}}
\newcommand{\lbhat}{\hat{\lb}}
\newcommand{\mbhat}{\hat{\mb}}
\newcommand{\nbhat}{\hat{\nb}}
\newcommand{\obhat}{\hat{\ob}}
\newcommand{\pbhat}{\hat{\pb}}
\newcommand{\qbhat}{\hat{\qb}}
\newcommand{\rbhat}{\hat{\rb}}
\newcommand{\sbhat}{\hat{\sb}}
\newcommand{\tbhat}{\hat{\tb}}
\newcommand{\ubhat}{\hat{\ub}}
\newcommand{\vbhat}{\hat{\vb}}
\newcommand{\wbhat}{\hat{\wb}}
\newcommand{\xbhat}{\hat{\xb}}
\newcommand{\ybhat}{\hat{\yb}}
\newcommand{\zbhat}{\hat{\zb}}

\newcommand{\Atil}{\tilde{A}}
\newcommand{\Btil}{\tilde{B}}
\newcommand{\Ctil}{\tilde{C}}
\newcommand{\Dtil}{\tilde{D}}
\newcommand{\Etil}{\tilde{E}}
\newcommand{\Ftil}{\tilde{F}}
\newcommand{\Gtil}{\tilde{G}}
\newcommand{\Htil}{\tilde{H}}
\newcommand{\Itil}{\tilde{I}}
\newcommand{\Jtil}{\tilde{J}}
\newcommand{\Ktil}{\tilde{K}}
\newcommand{\Ltil}{\tilde{L}}
\newcommand{\Mtil}{\tilde{M}}
\newcommand{\Ntil}{\tilde{N}}
\newcommand{\Otil}{\tilde{O}}
\newcommand{\Ptil}{\tilde{P}}
\newcommand{\Qtil}{\tilde{Q}}
\newcommand{\Rtil}{\tilde{R}}
\newcommand{\Stil}{\tilde{S}}
\newcommand{\Ttil}{\tilde{T}}
\newcommand{\Util}{\tilde{U}}
\newcommand{\Vtil}{\tilde{V}}
\newcommand{\Wtil}{\tilde{W}}
\newcommand{\Xtil}{\tilde{X}}
\newcommand{\Ytil}{\tilde{Y}}
\newcommand{\Ztil}{\tilde{Z}}

\newcommand{\abar}{\bar{a}}
\newcommand{\bbar}{\bar{b}}
\newcommand{\cbar}{\bar{c}}
\newcommand{\dbar}{\bar{d}}
\newcommand{\ebar}{\bar{e}}
\newcommand{\fbar}{\bar{f}}
\newcommand{\gbar}{\bar{g}}
\newcommand{\hbr}{\bar{h}}
\newcommand{\ibar}{\bar{i}}
\newcommand{\jbar}{\bar{j}}
\newcommand{\kbar}{\bar{k}}
\newcommand{\lbar}{\bar{l}}
\newcommand{\mbar}{\bar{m}}
\newcommand{\nbar}{\bar{n}}
\newcommand{\obar}{\bar{o}}
\newcommand{\pbar}{\bar{p}}
\newcommand{\qbar}{\bar{q}}
\newcommand{\rbar}{\bar{r}}
\newcommand{\sbar}{\bar{s}}
\newcommand{\tbar}{\bar{t}}
\newcommand{\ubar}{\bar{u}}
\newcommand{\vbar}{\bar{v}}
\newcommand{\wbar}{\bar{w}}
\newcommand{\xbar}{\bar{x}}
\newcommand{\ybar}{\bar{y}}
\newcommand{\zbar}{\bar{z}}

\newcommand{\abbar}{\bar{\ab}}
\newcommand{\bbbar}{\bar{\bb}}
\newcommand{\cbbar}{\bar{\cb}}
\newcommand{\dbbar}{\bar{\db}}
\newcommand{\ebbar}{\bar{\eb}}
\newcommand{\fbbar}{\bar{\fb}}
\newcommand{\gbbar}{\bar{\gb}}
\newcommand{\hbbar}{\bar{\hb}}
\newcommand{\ibbar}{\bar{\ib}}
\newcommand{\jbbar}{\bar{\jb}}
\newcommand{\kbbar}{\bar{\kb}}
\newcommand{\lbbar}{\bar{\lb}}
\newcommand{\mbbar}{\bar{\mb}}
\newcommand{\nbbar}{\bar{\nbb}}
\newcommand{\obbar}{\bar{\ob}}
\newcommand{\pbbar}{\bar{\pb}}
\newcommand{\qbbar}{\bar{\qb}}
\newcommand{\rbbar}{\bar{\rb}}
\newcommand{\sbbar}{\bar{\sbb}}
\newcommand{\tbbar}{\bar{\tb}}
\newcommand{\ubbar}{\bar{\ub}}
\newcommand{\vbbar}{\bar{\vb}}
\newcommand{\wbbar}{\bar{\wb}}
\newcommand{\xbbar}{\bar{\xb}}
\newcommand{\ybbar}{\bar{\yb}}
\newcommand{\zbbar}{\bar{\zb}}

\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sbb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}

\newcommand{\Abtil}{\tilde{\Ab}}
\newcommand{\Bbtil}{\tilde{\Bb}}
\newcommand{\Cbtil}{\tilde{\Cb}}
\newcommand{\Dbtil}{\tilde{\Db}}
\newcommand{\Ebtil}{\tilde{\Eb}}
\newcommand{\Fbtil}{\tilde{\Fb}}
\newcommand{\Gbtil}{\tilde{\Gb}}
\newcommand{\Hbtil}{\tilde{\Hb}}
\newcommand{\Ibtil}{\tilde{\Ib}}
\newcommand{\Jbtil}{\tilde{\Jb}}
\newcommand{\Kbtil}{\tilde{\Kb}}
\newcommand{\Lbtil}{\tilde{\Lb}}
\newcommand{\Mbtil}{\tilde{\Mb}}
\newcommand{\Nbtil}{\tilde{\Nb}}
\newcommand{\Obtil}{\tilde{\Ob}}
\newcommand{\Pbtil}{\tilde{\Pb}}
\newcommand{\Qbtil}{\tilde{\Qb}}
\newcommand{\Rbtil}{\tilde{\Rb}}
\newcommand{\Sbtil}{\tilde{\Sbb}}
\newcommand{\Tbtil}{\tilde{\Tb}}
\newcommand{\Ubtil}{\tilde{\Ub}}
\newcommand{\Vbtil}{\tilde{\Vb}}
\newcommand{\Wbtil}{\tilde{\Wb}}
\newcommand{\Xbtil}{\tilde{\Xb}}
\newcommand{\Ybtil}{\tilde{\Yb}}
\newcommand{\Zbtil}{\tilde{\Zb}}

\newcommand{\Abar}{\bar{A}}
\newcommand{\Bbar}{\bar{B}}
\newcommand{\Cbar}{\bar{C}}
\newcommand{\Dbar}{\bar{D}}
\newcommand{\Ebar}{\bar{E}}
\newcommand{\Fbar}{\bar{F}}
\newcommand{\Gbar}{\bar{G}}
\newcommand{\Hbar}{\bar{H}}
\newcommand{\Ibar}{\bar{I}}
\newcommand{\Jbar}{\bar{J}}
\newcommand{\Kbar}{\bar{K}}
\newcommand{\Lbar}{\bar{L}}
\newcommand{\Mbar}{\bar{M}}
\newcommand{\Nbar}{\bar{N}}
\newcommand{\Obar}{\bar{O}}
\newcommand{\Pbar}{\bar{P}}
\newcommand{\Qbar}{\bar{Q}}
\newcommand{\Rbar}{\bar{R}}
\newcommand{\Sbar}{\bar{S}}
\newcommand{\Tbar}{\bar{T}}
\newcommand{\Ubar}{\bar{U}}
\newcommand{\Vbar}{\bar{V}}
\newcommand{\Wbar}{\bar{W}}
\newcommand{\Xbar}{\bar{X}}
\newcommand{\Ybar}{\bar{Y}}
\newcommand{\Zbar}{\bar{Z}}

\newcommand{\Abbar}{\bar{\Ab}}
\newcommand{\Bbbar}{\bar{\Bb}}
\newcommand{\Cbbar}{\bar{\Cb}}
\newcommand{\Dbbar}{\bar{\Db}}
\newcommand{\Ebbar}{\bar{\Eb}}
\newcommand{\Fbbar}{\bar{\Fb}}
\newcommand{\Gbbar}{\bar{\Gb}}
\newcommand{\Hbbar}{\bar{\Hb}}
\newcommand{\Ibbar}{\bar{\Ib}}
\newcommand{\Jbbar}{\bar{\Jb}}
\newcommand{\Kbbar}{\bar{\Kb}}
\newcommand{\Lbbar}{\bar{\Lb}}
\newcommand{\Mbbar}{\bar{\Mb}}
\newcommand{\Nbbar}{\bar{\Nb}}
\newcommand{\Obbar}{\bar{\Ob}}
\newcommand{\Pbbar}{\bar{\Pb}}
\newcommand{\Qbbar}{\bar{\Qb}}
\newcommand{\Rbbar}{\bar{\Rb}}
\newcommand{\Sbbar}{\bar{\Sb}}
\newcommand{\Tbbar}{\bar{\Tb}}
\newcommand{\Ubbar}{\bar{\Ub}}
\newcommand{\Vbbar}{\bar{\Vb}}
\newcommand{\Wbbar}{\bar{\Wb}}
\newcommand{\Xbbar}{\bar{\Xb}}
\newcommand{\Ybbar}{\bar{\Yb}}
\newcommand{\Zbbar}{\bar{\Zb}}

\newcommand{\Ahat}{\hat{A}}
\newcommand{\Bhat}{\hat{B}}
\newcommand{\Chat}{\hat{C}}
\newcommand{\Dhat}{\hat{D}}
\newcommand{\Ehat}{\hat{E}}
\newcommand{\Fhat}{\hat{F}}
\newcommand{\Ghat}{\hat{G}}
\newcommand{\Hhat}{\hat{H}}
\newcommand{\Ihat}{\hat{I}}
\newcommand{\Jhat}{\hat{J}}
\newcommand{\Khat}{\hat{K}}
\newcommand{\Lhat}{\hat{L}}
\newcommand{\Mhat}{\hat{M}}
\newcommand{\Nhat}{\hat{N}}
\newcommand{\Ohat}{\hat{O}}
\newcommand{\Phat}{\widehat{P}}
\newcommand{\Qhat}{\widehat{Q}}
\newcommand{\Rhat}{\hat{R}}
\newcommand{\Shat}{\widehat{S}}
\newcommand{\That}{\widehat{T}}
\newcommand{\Uhat}{\hat{U}}
\newcommand{\Vhat}{\hat{V}}
\newcommand{\What}{\hat{W}}
\newcommand{\Xhat}{\hat{X}}
\newcommand{\Yhat}{\hat{Y}}
\newcommand{\Zhat}{\hat{Z}}

\newcommand{\Abhat}{\hat{\Ab}}
\newcommand{\Bbhat}{\hat{\Bb}}
\newcommand{\Cbhat}{\hat{\Cb}}
\newcommand{\Dbhat}{\hat{\Db}}
\newcommand{\Ebhat}{\hat{\Eb}}
\newcommand{\Fbhat}{\hat{\Fb}}
\newcommand{\Gbhat}{\hat{\Gb}}
\newcommand{\Hbhat}{\hat{\Hb}}
\newcommand{\Ibhat}{\hat{\Ib}}
\newcommand{\Jbhat}{\hat{\Jb}}
\newcommand{\Kbhat}{\hat{\Kb}}
\newcommand{\Lbhat}{\hat{\Lb}}
\newcommand{\Mbhat}{\hat{\Mb}}
\newcommand{\Nbhat}{\hat{\Nb}}
\newcommand{\Obhat}{\hat{\Ob}}
\newcommand{\Pbhat}{\hat{\Pb}}
\newcommand{\Qbhat}{\hat{\Qb}}
\newcommand{\Rbhat}{\hat{\Rb}}
\newcommand{\Sbhat}{\hat{\Sb}}
\newcommand{\Tbhat}{\hat{\Tb}}
\newcommand{\Ubhat}{\hat{\Ub}}
\newcommand{\Vbhat}{\hat{\Vb}}
\newcommand{\Wbhat}{\hat{\Wb}}
\newcommand{\Xbhat}{\hat{\Xb}}
\newcommand{\Ybhat}{\hat{\Yb}}
\newcommand{\Zbhat}{\hat{\Zb}}

\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{{\mathcal{S}}}
\newcommand{\Tcal}{{\mathcal{T}}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}

\newcommand{\Atilde}{\widetilde{A}}
\newcommand{\Btilde}{\widetilde{B}}
\newcommand{\Ctilde}{\widetilde{C}}
\newcommand{\Dtilde}{\widetilde{D}}
\newcommand{\Etilde}{\widetilde{E}}
\newcommand{\Ftilde}{\widetilde{F}}
\newcommand{\Gtilde}{\widetilde{G}}
\newcommand{\Htilde}{\widetilde{H}}
\newcommand{\Itilde}{\widetilde{I}}
\newcommand{\Jtilde}{\widetilde{J}}
\newcommand{\Ktilde}{\widetilde{K}}
\newcommand{\Ltilde}{\widetilde{L}}
\newcommand{\Mtilde}{\widetilde{M}}
\newcommand{\Ntilde}{\widetilde{N}}
\newcommand{\Otilde}{\widetilde{O}}
\newcommand{\Ptilde}{\widetilde{P}}
\newcommand{\Qtilde}{\widetilde{Q}}
\newcommand{\Rtilde}{\widetilde{R}}
\newcommand{\Stilde}{\widetilde{S}}
\newcommand{\Ttilde}{\widetilde{T}}
\newcommand{\Utilde}{\widetilde{U}}
\newcommand{\Vtilde}{\widetilde{V}}
\newcommand{\Wtilde}{\widetilde{W}}
\newcommand{\Xtilde}{\widetilde{X}}
\newcommand{\Ytilde}{\widetilde{Y}}
\newcommand{\Ztilde}{\widetilde{Z}}

\renewcommand{\vec}[1]{\mathbf{\boldsymbol{#1}}}

\newcommand{\avec}{\vec{a}}
\newcommand{\bvec}{\vec{b}}
\newcommand{\cvec}{\vec{c}}
\newcommand{\dvec}{\vec{d}}
\newcommand{\evec}{\vec{e}}
\newcommand{\fvec}{\vec{f}}
\newcommand{\gvec}{\vec{g}}
\newcommand{\hvec}{\vec{h}}
\newcommand{\ivec}{\vec{i}}
\newcommand{\jvec}{\vec{j}}
\newcommand{\kvec}{\vec{k}}
\newcommand{\lvec}{\vec{l}}
\newcommand{\mvec}{\vec{m}}
\newcommand{\nvec}{\vec{n}}
\newcommand{\ovec}{\vec{o}}
\newcommand{\pvec}{\vec{p}}
\newcommand{\qvec}{\vec{q}}
\newcommand{\rvec}{\vec{r}}
\newcommand{\svec}{\vec{s}}
\newcommand{\tvec}{\vec{t}}
\newcommand{\uvec}{\vec{u}}
\newcommand{\vvec}{\vec{v}}
\newcommand{\wvec}{\vec{w}}
\newcommand{\xvec}{\vec{x}}
\newcommand{\yvec}{\vec{y}}
\newcommand{\zvec}{\vec{z}}

\newcommand{\epsilonvec}{\vec{\epsilon}}
\newcommand{\vepsilon}{\vec{\epsilon}}
\newcommand{\zerovec}{\vec{0}}
\newcommand{\onevec}{\vec{1}}
\newcommand{\eye}{I}

\newcommand{\va}{\vec{a}}
\newcommand{\vecb}{\vec{b}}
\newcommand{\vc}{\vec{c}}
\newcommand{\vd}{\vec{d}}
\newcommand{\veee}{\vec{e}}
\newcommand{\vf}{\vec{f}}
\newcommand{\vg}{\vec{g}}
\newcommand{\vh}{\vec{h}}
\newcommand{\vi}{\vec{i}}
\newcommand{\vk}{\vec{k}}
\newcommand{\vl}{\vec{l}}
\newcommand{\vm}{\vec{m}}
\newcommand{\vn}{\vec{n}}
\newcommand{\vo}{\vec{o}}
\newcommand{\vp}{\vec{p}}
\newcommand{\vq}{\vec{q}}
\newcommand{\vr}{\vec{r}}
\newcommand{\vs}{\vec{s}}
\newcommand{\vt}{\vec{t}}
\newcommand{\vu}{\vec{u}}
\newcommand{\vv}{\vec{v}}
\newcommand{\vw}{\vec{w}}
\newcommand{\vx}{\vec{x}}
\newcommand{\vy}{\vec{y}}
\newcommand{\vz}{\vec{z}}

\newcommand{\Avec}{\vec{A}}
\newcommand{\Bvec}{\vec{B}}
\newcommand{\Cvec}{\vec{C}}
\newcommand{\Dvec}{\vec{D}}
\newcommand{\Evec}{\vec{E}}
\newcommand{\Fvec}{\vec{F}}
\newcommand{\Gvec}{\vec{G}}
\newcommand{\Hvec}{\vec{H}}
\newcommand{\Ivec}{\vec{I}}
\newcommand{\Jvec}{\vec{J}}
\newcommand{\Kvec}{\vec{K}}
\newcommand{\Lvec}{\vec{L}}
\newcommand{\Mvec}{\vec{M}}
\newcommand{\Nvec}{\vec{N}}
\newcommand{\Ovec}{\vec{O}}
\newcommand{\Pvec}{\vec{P}}
\newcommand{\Qvec}{\vec{Q}}
\newcommand{\Rvec}{\vec{R}}
\newcommand{\Svec}{\vec{S}}
\newcommand{\Tvec}{\vec{T}}
\newcommand{\Uvec}{\vec{U}}
\newcommand{\Vvec}{\vec{V}}
\newcommand{\Wvec}{\vec{W}}
\newcommand{\Xvec}{\vec{X}}
\newcommand{\Yvec}{\vec{Y}}
\newcommand{\Zvec}{\vec{Z}}

\newcommand{\Amat}{\Ab}
\newcommand{\Bmat}{\Bb}
\newcommand{\Cmat}{\Cb}
\newcommand{\Dmat}{\Db}
\newcommand{\Emat}{\Eb}
\newcommand{\Fmat}{\Fb}
\newcommand{\Gmat}{\Gb}
\newcommand{\Hmat}{\Hb}
\newcommand{\Imat}{\Ib}

\newcommand{\Vmat}{\Vb}
\newcommand{\Wmat}{\Wb}
\newcommand{\Xmat}{\Xb}
\newcommand{\Ymat}{\Yb}
\newcommand{\Zmat}{\Zb}


\newcommand{\yvecbar}{\bar{\vec{y}}}
\newcommand{\wvecbar}{\bar{\vec{w}}}
\newcommand{\xvecbar}{\bar{\vec{x}}}
\newcommand{\yvectil}{\tilde{\vec{y}}}
\newcommand{\yvechat}{\hat{\vec{y}}}


%%%%%%%% Theorems and Friends %%%%%%%%%%%%%%%

%% Some style files might actually define these variables.
%% So don't mess with them if they are already defined

\ifx\BlackBox\undefined
\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\fi

\ifx\QED\undefined
\def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
\fi

\newcommand{\eproof}{$\null\hfill\blacksquare$}
\ifx\proof\undefined
\newenvironment{proof}{\par\noindent{\bf Proof:\ }}{\hfill\BlackBox\\[2mm]}
\else
\renewenvironment{proof}{\par\noindent{\bf Proof:\ }}{\eproof} %{\hfill\BlackBox\\[.3mm]}
\newenvironment{proofsketch}{\par\noindent{\bf Proof Sketch:\ }}{\eproof} %{\hfill\BlackBox\\[.3mm]}
\fi

\ifx\theorem\undefined
\newtheorem{theorem}{Theorem}
\fi

\ifx\example\undefined
\newtheorem{example}{Example}
\fi

\ifx\property\undefined
\newtheorem{property}{Property}
\fi

\ifx\lemma\undefined
\newtheorem{lemma}[theorem]{Lemma}
\fi

\ifx\proposition\undefined
\newtheorem{proposition}[theorem]{Proposition}
\fi

\ifx\remark\undefined
\newtheorem{remark}[theorem]{Remark}
\fi

\ifx\corollary\undefined
\newtheorem{corollary}[theorem]{Corollary}
\fi

\ifx\definition\undefined
\newtheorem{definition}{Definition}
\fi

\ifx\conjecture\undefined
\newtheorem{conjecture}[theorem]{Conjecture}
\fi

\ifx\axiom\undefined
\newtheorem{axiom}[theorem]{Axiom}
\fi

\ifx\claim\undefined
\newtheorem{claim}[theorem]{Claim}
\fi

\ifx\assumption\undefined
\newtheorem{assumption}[theorem]{Assumption}
\fi

% \renewcommand{\qedsymbol}{$\blacksquare$}


%%%%%%%% Widely accepted Sets and Symbols %%%%%%%%%%%%%%%

\newcommand{\CC}{\mathbb{C}} % Complex numbers
\newcommand{\EE}{\mathbb{E}} % Expectation
\newcommand{\FF}{\mathbb{F}} % Fexpectation
\newcommand{\HH}{\mathbb{H}} % Arbitrary field
\newcommand{\II}{\mathbb{I}} % Delta Indicator
\newcommand{\KK}{\mathbb{K}} % Arbitrary field
\newcommand{\MM}{\mathbb{M}} % Median
\newcommand{\NN}{\mathbb{N}} % Natural numbers
\newcommand{\PP}{\mathbb{P}} % Probability
\newcommand{\QQ}{\mathbb{Q}} % Rationals
\newcommand{\RR}{\mathbb{R}} % Real numbers
\newcommand{\RRbar}{\overline{\RR}} % Real numbers
\newcommand{\VV}{\mathbb{V}} % Variance
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}} % Integers

%%%%%%%% Mathematical Operations %%%%%%%%%%%%%%%

\newcommand*{\mini}{\mathop{\mathrm{minimize}}}
\newcommand*{\maxi}{\mathop{\mathrm{maximize}}}
\newcommand*{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand*{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand*{\arginf}{\mathop{\mathrm{arginf}}}
\newcommand*{\argsup}{\mathop{\mathrm{argsup}}}
\newcommand{\sgn}{\mathop{\mathrm{sign}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\spec}{\mathop{\mathrm{sp}}}
\newcommand{\te}{\mathop{\mathrm{te}}}
\newcommand{\diag}{\mathop{\mathrm{diag}}}
\newcommand{\rank}{\mathop{\mathrm{rank}}}
\newcommand{\vect}{\mathop{\mathrm{vec}}}
\newcommand{\traj}{\mathop{\mathrm{Traj}}}
\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\const}{\mathrm{constant}}
\newcommand{\dom}{\mathop{\mathrm{dom}}}
\newcommand{\ri}{\mathop{\mathrm{ri}}}
\newcommand{\cl}{\mathop{\mathrm{cl}}}
\newcommand{\intr}{\mathop{\mathrm{int}}}
\newcommand{\bd}{\mathop{\mathrm{bd}}}
\newcommand{\emp}{\mathop{\mathrm{emp}}}
\newcommand{\core}{\mathop{\mathrm{core}}}
\newcommand{\co}{\mathop{\mathrm{co}}}
\newcommand{\nnz}{\mathop{\mathrm{nnz}}}

%\newcommand{\ln}{\mathop{\mathrm{ln}}}
%%%%%%%% Utility functions %%%%%%%%%%%%%%%

\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}
\newcommand{\mychoose}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\newcommand{\mydet}[1]{\det\left[ #1 \right]}
\newcommand{\myspan}[1]{\mathrm{span}\cbr{#1}}
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}
\newcommand{\pwrt}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ppwrt}[1]{\frac{\partial^2}{(\partial #1)^2}}
\newcommand{\aleq}{\preccurlyeq}
\newcommand{\ageq}{\succcurlyeq}
%%%%%%%% Short Forms %%%%%%%%%%%%%%%

\newcommand{\ea}{\emph{et al.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\iid}{{{i.i.d.} }}
%\newcommand{\iid}{{\emph{iid} }}
\newcommand{\iidn}{{\emph{iid}}}
\newcommand{\cf}{\emph{cf.}\ }
\newcommand{\wrt}{\emph{w.r.t.}\ }

%%%%%%%% Brackets %%%%%%%%%%%%%%%

\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\ccc}[1]{|\!|\!|#1|\!|\!|}
\newcommand{\sembrack}[1]{[\![#1]\!]}

%%%%%%%%%%%%%%%  Mathematical Constants  %%%%%%%%%%%%%%%

\newcommand{\one}{\mathbf{1}}  % Identity
\newcommand{\zero}{\mathbf{0}} % Zero
\newcommand{\ind}{\boldsymbol{\mathsf{I}}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\sqrttwo}{\sqrt{2}}
\newcommand{\invsqrttwo}{\frac{1}{\sqrt{2}}}
\newcommand{\rmd}{\ensuremath{\mathrm{d}}}

%%%%%%%% Greek Symbols %%%%%%%%%%%%%%%

\newcommand{\sigmab}{\bm{\sigma}}
\newcommand{\Sigmab}{\mathbf{\Sigma}}

\newcommand{\valpha}{\vec{\alpha}}
\newcommand{\val}{\vec{\alpha}}
\newcommand{\vbeta}{\vec{\beta}}
\newcommand{\vdelta}{\vec{\delta}}
\newcommand{\vgamma}{\vec{\gamma}}
\newcommand{\vsigma}{\vec{\sigma}}
\newcommand{\vtheta}{\vec{\theta}}
\newcommand{\veta}{\vec{\eta}}
\newcommand{\vnu}{\vec{\nu}}
\newcommand{\vpsi}{\vec{\psi}}
\newcommand{\vpi}{\vec{\pi}}
\newcommand{\vphi}{\vec{\phi}}
\newcommand{\vvarphi}{\vec{\varphi}}
\newcommand{\vxi}{\vec{\xi}}
\newcommand{\vzeta}{\vec{\zeta}}

\newcommand{\valbar}{\bar{\val}}
\newcommand{\valhat}{\hat{\val}}
\newcommand{\valtil}{\tilde{\val}}
\newcommand{\vthtil}{\tilde{\vth}}
\newcommand{\vthhat}{\hat{\vth}}
\newcommand{\vthbar}{\bar{\vth}}
\newcommand{\vbetatil}{\tilde{\vbeta}}
\newcommand{\vbetahat}{\hat{\vbeta}}

\newcommand{\alphavec}{\val}
\newcommand{\alphavecbar}{\bar{\val}}
\newcommand{\alphavechat}{\hat{\val}}
\newcommand{\alphavectil}{\tilde{\val}}
\newcommand{\betavec}{\vec{\beta}}
\newcommand{\gammavec}{\vec{\gamma}}
\newcommand{\deltavec}{\vec{\delta}}
\newcommand{\etavec}{\vec{\eta}}
\newcommand{\phivec}{\vec{\phi}}
\newcommand{\psivec}{\vec{\psi}}
\newcommand{\thetavec}{\vec{\theta}}
\newcommand{\muvec}{\vec{\mu}}
\newcommand{\xivec}{\vec{\xi}}
\newcommand{\chivec}{\vec{\chi}}
\newcommand{\lambdavec}{\vec{\lambda}}

\newcommand{\alphab}{\boldsymbol{\alpha}}
\newcommand{\betab}{\boldsymbol{\beta}}
\newcommand{\gammab}{\boldsymbol{\gamma}}
\newcommand{\thetab}{\boldsymbol{\theta}}
\newcommand{\mub}{\boldsymbol{\mu}}
\newcommand{\xib}{\boldsymbol{\xi}}
\newcommand{\Deltab}{\boldsymbol{\Delta}}
\newcommand{\Pib}{\boldsymbol{\Pi}}
\newcommand{\etab}{\boldsymbol{\eta}}
\newcommand{\taub}{\boldsymbol{\tau}}
\newcommand{\lambdab}{\boldsymbol{\lambda}}
\newcommand{\pitil}{\tilde{\pi}}
\newcommand{\elltil}{\tilde{\ell}}
\newcommand{\rhob}{\boldsymbol{\rho}}

\newcommand{\delhat}{\hat{\delta}}
\newcommand{\phihat}{\hat{\phi}}
\newcommand{\delbar}{\bar{\delta}}
\newcommand{\alphahat}{\hat{\alpha}}
\newcommand{\alphatil}{\tilde{\alpha}}
\newcommand{\mubar}{\bar{\mu}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\thetabar}{\bar{\theta}}
\newcommand{\betahat}{\hat{\beta}}

\newcommand{\xibar}{\bar{\xi}}
\newcommand{\lambdavectil}{\tilde{\vec{\lambda}}}
\newcommand{\thetatil}{\tilde{\theta}}
\newcommand{\betatil}{\tilde{\beta}}

%%%%%%%% Various Optimizers %%%%%%%%%%%%%%%

\newcommand{\BMRM}{{\sf BMRM}}
\newcommand{\bmrm}{{\sf BMRM}}
\newcommand{\cpm}{{\sf CPM}}
\newcommand{\liblinear}{{\sf liblinear}}
\newcommand{\lsbmrm}{{\sf ls-bmrm}}
\newcommand{\qpbmrm}{{\sf qp-bmrm}}
\newcommand{\pegasos}{{\sf pegasos}}
\newcommand{\pegan}{{\sf pegasos-$n$}}
\newcommand{\pegaone}{{\sf pegasos-1}}
\newcommand{\svmstruct}{{\sf SVM-Struct}}
\newcommand{\svmperf}{{\sf SVM-Perf}}
\newcommand{\nest}{{\sf pragam}}
\newcommand{\nestb}{{\sf pragam-b}}
\newcommand{\mcn}{{\sf M$^3$N}}
\newcommand{\expgrad}{{\sf ExpGrad}}
\newcommand{\smo}{{\sf SMO}}
\newcommand{\lasvm}{{\sf LaSVM}}
\newcommand{\sms}{{\sf SMS}}


\newcommand{\prbep}{{\sf PRBEP}}
\newcommand{\rocarea}{{\sf ROCArea}}

\newcommand{\arow}[2]{#1_{#2\cdot}}
\newcommand{\acol}[2]{#1_{\cdot#2}}
\newcommand{\expunder}[1]{\mathop{\EE}\limits_{#1}}
\newcommand{\mean}[1]{\mathop{\EE}\sbr{{#1}}}
\newcommand{\vars}[2]{\var_{{#1}}\sbr{{#2}}}
\newcommand{\expec}[2]{\mathop{\EE}_{{#1}}\sbr{{#2}}}

\newcommand{\twoco}[1]{\multicolumn{2}{c|}{#1}}
\def\ci{\perp\!\!\!\perp}

\newcommand{\ve}{\varepsilon}

\newcommand{\gstar}{g^{\star}}
\newcommand{\fstar}{f^{\star}}
\newcommand{\hstar}{h^{\star}}
\newcommand{\Astar}{A^{\star}}
\newcommand{\Kstar}{K^{\star}}

\newcommand{\var}{\mathrm{Var}}
\newcommand{\grad}{{\nabla}}
\newcommand{\gradtil}{{\tilde{\grad}}}
\newcommand{\MED}{{\text{MED}}}
\newcommand{\where}{{\quad \text{where} \quad}}
\newcommand{\lcg}{{\textit{l.c.g}}}
\newcommand{\cp}{\mathrm{cp}}
\newcommand{\err}{{\sf err}}
\newcommand{\wvechat}{\hat{\vec{w}}}

\newcommand{\ydiff}[2]{\delta(#1, #2)}
\newcommand{\ykdiff}[2]{\delta(#1, #2)^{\kappa}}
\newcommand{\myfdiff}[2]{\Delta f(#1, #2)}


\newcommand{\Aone}{\textbf{A1}}
\newcommand{\Atwo}{\textbf{A2}}


==> sections/tmp.tex <==
\section{Direct Optimization without Surrogates}

Consider the follow problem ($\zvec=\gvec_h/\tau$ recovers the original problem):
\[
\min_{\alphavec\in\Delta}\quad 
\langle \zvec,\alphavec\rangle + \|\alphavec\|_2
\]
We now derive its dual problem.
The Lagrangian function is
\[
\Lambda(\alphavec,\lambdavec,\nu)
= \zvec^\top \alphavec + \|\alphavec\|_2
- \lambdavec^\top \alphavec + \nu (1-\onevec^\top\alphavec)
\qquad
\nu\in\RR,\lambdavec\succeq0
\]
Taking derivative w.r.t. $\alphavec$ and setting it to zero gives
\[
\frac{\partial\Lambda}{\partial\alphavec}
= \zvec + \alphavec/\|\alphavec\|_2
-\lambdavec-\nu\onevec = 0
\Longrightarrow 
\alphavec^*/\|\alphavec^*\|_2 
= \lambdavec + \nu\onevec - \zvec.
\]
Notice that $\alphavec\neq\zerovec$ so we have the constraint $\|\lambdavec+\nu\onevec-\zvec\|_2=1$.
Use this $\alphavec^*$ in $\Lambda$ gives the following dual problem
\[
\max_{\nu,\lambdavec}\quad \nu
\qquad
\text{s.t.}
\quad \|\lambdavec+\nu\onevec-\zvec\|_2=1
\quad\text{and}\quad
\lambdavec\succeq0
\]
We would like to increase $\nu$ as much as possible, and the maximum we can attain is $\nu^*$ satisfying $\|[\nu^*\onevec-\zvec]_+\|_2=1$ where $[\zvec]_+=\max(\zerovec,\zvec)$. 
In this case, the optimal $\lambdavec^*$ can be attained as $\lambda^*_i=0$ if $z_i-\nu^*<0$, otherwise $\lambda^*_i=z_i-\nu^*$.
Although we do not have a closed-form expression for the optimal $\nu^*$, we can use binary search to find it, starting from the interval $[z_{\min},z_{\max}+1]$.
Then we can recover the primal solution as
\begin{equation}
\alphavec^*=[\nu^*\onevec-\zvec]_+
/\|[\nu^*\onevec-\zvec]_+\|_1.
\label{eq:sharpmax}
\end{equation}
This procedure is pictorially demonstrated in \cref{fig:original_sol}. 
\cref{eq:sharpmax} gives rise to a novel way to project any vector $\zvec$ to the probability simplex, which is of independent interest and may be used in some other contexts\footnote{For example, if we consider $-\zvec$ to be the logits of the final classification layer of a neural network, this projection provides another way to produce class probabilities similar to the softmax transformation.}.
To use this transformation in a neural network with gradient-based optimizer, however, we need to calculate its Jacobian $J_{ij}=\partial\alpha_i/\partial z_j$, which is involved due to the $\nu^*$.
In the following, we show how to compute the Jacobian.


\begin{figure}
  \centering
  \includegraphics[width=0.5\textwidth]{figures/original_sol.png}
  \caption{Solution to the original problem (best viewed in color). $\lambda^*$ compensates whatever is above the $\nu^*$, while $\nu^*$ is chosen such that the vector of the green bars has $L_2$ norm of 1.}
  \label{fig:original_sol}
\end{figure}


Let $S=\{i|\nu-z_i>0\}$ be the support of the probability vector $\alphavec$. 
$J_{ij}=0$ if $i\notin S$ or $j\notin S$ since $\alpha_i=0$ in the former case while $z_j$ does not contribute to the $\alphavec$ in the latter case.
Now consider the case $i,j\in S$.
Let $K=\|[\nu\onevec-\zvec]_+\|_1=\sum_{j\in S}(\nu-z_j)$.
Then $\alpha_i=(\nu-z_i)\cdot \frac{1}{K}$ and
\begin{equation}
\frac{\partial\alpha_i}{\partial z_j}
=\left(\frac{\partial\nu}{\partial z_j}-\delta_{i=j}\right)
\cdot\frac{1}{K}
-\frac{1}{K^2}
\cdot\frac{\partial K}{\partial z_j}
\cdot(\nu-z_i)
=\frac{1}{K}\left(\frac{\partial\nu}{\partial z_j}-\delta_{i=j}
-\frac{\partial K}{\partial z_j}\cdot\alpha_i\right),
\label{eq:alpha_i_z_j_nu_K}
\end{equation}
where $\delta_{i=j}$ is the indicator or delta function.
Now we compute $\frac{\partial\nu}{\partial z_j}$ and $\frac{\partial K}{\partial z_j}$.
By the definition of $\nu$, we know that
\[
\begin{split}
\sum_{j\in S} (\nu-z_j)^2
&=|S|\nu^2-2\nu\sum_{j\in S} z_j+\sum_{j\in S}z_j^2
=1\\
\Longrightarrow
\nu&=\frac{\sum_{j\in S}z_j}{|S|}
+\frac{\sqrt{A}}{|S|}
\quad\text{where}\quad
A=\left(\sum_{j\in S}z_j\right)^2
-|S|\left(\sum_{j\in S}z_j^2-1\right)\\
\Longrightarrow
\frac{\partial \nu}{\partial z_j}
&=\frac{1}{|S|}
+\frac{B_j}{|S|\sqrt{A}}
\quad\text{where}\quad
B_j=\sum_{j'\in S}z_{j'}-|S|z_j
\end{split}
\]
% https://math.stackexchange.com/a/439238
The first right-arrow is due to the quadratic formula and realizing that $\sum_{j\in S}z_j/|S|$ is the mean of the supported $z_j$ so $\nu$ must be bigger than it (i.e., we take $+$ in the $\pm$ of the quadratic formula, otherwise some of the $z_j$ will not be in the support anymore). 
And
\[
\frac{\partial K}{\partial z_j} 
= |S|\cdot\frac{\partial\nu}{\partial z_j} - 1
= \frac{B_j}{\sqrt{A}}.
\]
Plugging these in \cref{eq:alpha_i_z_j_nu_K} gives
\[
\frac{\partial\alpha_i}{\partial z_j}
=\frac{1}{K}
\left[
\frac{1}{|S|}-\delta_{i=j}
+\frac{B_j}{\sqrt{A}}
\cdot\left(\frac{1}{|S|}-\alpha_i\right)
\right]
\]
Note that
\[
\frac{B_j}{K}=\frac{\sum_{j'\in S}z_{j'}-|S|z_j}
{\sum_{j'\in S}(\nu-z_{j'})}
=\frac{\sum_{j'\in S}(z_{j'}-\nu)+|S|(\nu-z_j)}
{\sum_{j'\in S}(\nu-z_{j'})}
=|S|\alpha_j-1.
\]
Then
\[
J_{ij}
=\frac{\partial\alpha_i}{\partial z_j}
=\frac{1}{K}\left(\frac{1}{|S|}-\delta_{i=j}\right)
-\frac{|S|}{\sqrt{A}}
\left(\alpha_i-\frac{1}{|S|}\right)
\left(\alpha_j-\frac{1}{|S|}\right).
\]
We can do a sanity check by noticing that
\[
\sum_i\frac{\partial\alpha_i}{\partial z_j}
=\frac{\partial\sum_i\alpha_i}{\partial z_j}
=\frac{\partial 1}{\partial z_j}=0.
\]
In matrix form,
\[
J=\frac{1}{K}
\left(\frac{\svec\svec^\top}{|S|}-\Diag(\svec)\right)
-\frac{|S|}{\sqrt{A}}
\left(\alphavec\circ\svec-\frac{\svec}{|S|}\right)
\left(\alphavec\circ\svec-\frac{\svec}{|S|}\right)^\top,
\]
where $s_i=\delta_{i\in S}$ and $\circ$ is element-wise multiplication. 
More often, we need to compute its multiplication with a vector $\vvec$
\[
J\vvec=
\frac{\svec}{K}\circ\left(\frac{\svec^\top\vvec}{|S|}
-\vvec\right)
-\frac{|S|}{\sqrt{A}}
\left(\alphavec\circ\svec-\frac{\svec}{|S|}\right)
\left(\alphavec\circ\svec-\frac{\svec}{|S|}\right)^\top
\vvec.
\]
Note that all quantities except $A$ have been computed during the forward pass of calculating \cref{eq:sharpmax}.
$A$ can be computed in $O(|S|)$ time so the overall computation is still $O(|S|)$.

[Other properties when $-\zvec$ is considered as logits.]

Case of 2d $[z,0]$. 
\[
\begin{split}
A&=z^2-2(z^2-1)=2-z^2\\
\nu&=\frac{-z+\sqrt{2-z^2}}{2}\\
K&=2\nu+z=\sqrt{2-z^2}\\
\alpha&=(\nu+z)/K=\frac{1}{2}+\frac{z}{2\sqrt{2-z^2}}
\end{split}
\]





% \subsection{Further upper bound}
% https://en.wikipedia.org/wiki/R%C3%A9nyi_entropy#Inequalities_between_different_values_of_%CE%B1
% https://en.wikipedia.org/wiki/Pinsker%27s_inequality
% https://en.wikipedia.org/wiki/Total_variation_distance_of_probability_measures
% https://en.wikipedia.org/wiki/Lambert_W_function
% Here we upper bound the $\|\alpha\|_2$.
% The Pinsker's Inequality says both the following
% \[
% \begin{split}
% \sqrt{\frac{1}{2}KL(\alpha\|u)}
% &\ge\frac{1}{2}\|\alpha-u\|_1
% \ge\frac{1}{2}\|\alpha-u\|_2\\
% \sqrt{\frac{1}{2}KL(\alpha\|u)}
% &\ge\|\alpha-u\|_\infty
% \ge\frac{1}{\sqrt{k}}\|\alpha-u\|_2
% \end{split}
% \]
% We pick $u$ to be uniform. 
% Combining the two gives the following
% \[
% \|\alpha\|_2\le
% \sqrt{\min\{k/2,2\}(\alpha\cdot \log \alpha
% +\log k) + 1/k}
% \]



% \subsection{For $L_2$ Regression}
% \begin{itemize}
% \item Loss is $L_2$
% \item Matching $M_P,M_Q$ in some layer, no reweighting, mini-batch
% \item Power iteration for a few steps, back-prop through
% \item Can work with multiple source domains
% \end{itemize}





\section{Jacobian}
\label{appendix:jac}

[TODO: for now it is based on $\zvec$, need to change to $-\zvec$.]

Here we calculate the Jacobian $J_{ij}=\partial\alpha_i/\partial z_j$.
% To use this transformation in a neural network with gradient-based optimizer, however, we need to calculate its Jacobian $J_{ij}=\partial\alpha_i/\partial z_j$, which is involved due to the $\nu^*$.
% In the following, we show how to compute the Jacobian.

Let $S=\{i|\nu-z_i>0\}$ be the support of the probability vector $\alphavec$. 
$J_{ij}=0$ if $i\notin S$ or $j\notin S$ since $\alpha_i=0$ in the former case while $z_j$ does not contribute to the $\alphavec$ in the latter case.
Now consider the case $i,j\in S$.
Let $K=\|[\nu\onevec-\zvec]_+\|_1=\sum_{j\in S}(\nu-z_j)$.
Then $\alpha_i=(\nu-z_i)\cdot \frac{1}{K}$ and
\begin{equation}
\frac{\partial\alpha_i}{\partial z_j}
=\left(\frac{\partial\nu}{\partial z_j}-\delta_{i=j}\right)
\cdot\frac{1}{K}
-\frac{1}{K^2}
\cdot\frac{\partial K}{\partial z_j}
\cdot(\nu-z_i)
=\frac{1}{K}\left(\frac{\partial\nu}{\partial z_j}-\delta_{i=j}
-\frac{\partial K}{\partial z_j}\cdot\alpha_i\right),
\label{eq:alpha_i_z_j_nu_K}
\end{equation}
where $\delta_{i=j}$ is the indicator or delta function.
Now we compute $\frac{\partial\nu}{\partial z_j}$ and $\frac{\partial K}{\partial z_j}$.
By the definition of $\nu$, we know that
\[
\begin{split}
\sum_{j\in S} (\nu-z_j)^2
&=|S|\nu^2-2\nu\sum_{j\in S} z_j+\sum_{j\in S}z_j^2
=1\\
\Longrightarrow
\nu&=\frac{\sum_{j\in S}z_j}{|S|}
+\frac{\sqrt{A}}{|S|}
\quad\text{where}\quad
A=\left(\sum_{j\in S}z_j\right)^2
-|S|\left(\sum_{j\in S}z_j^2-1\right)\\
\Longrightarrow
\frac{\partial \nu}{\partial z_j}
&=\frac{1}{|S|}
+\frac{B_j}{|S|\sqrt{A}}
\quad\text{where}\quad
B_j=\sum_{j'\in S}z_{j'}-|S|z_j
\end{split}
\]
% https://math.stackexchange.com/a/439238
The first right-arrow is due to the quadratic formula and realizing that $\sum_{j\in S}z_j/|S|$ is the mean of the supported $z_j$ so $\nu$ must be bigger than it (i.e., we take $+$ in the $\pm$ of the quadratic formula, otherwise some of the $z_j$ will not be in the support anymore). 
And
\[
\frac{\partial K}{\partial z_j} 
= |S|\cdot\frac{\partial\nu}{\partial z_j} - 1
= \frac{B_j}{\sqrt{A}}.
\]
Plugging these in \cref{eq:alpha_i_z_j_nu_K} gives
\[
\frac{\partial\alpha_i}{\partial z_j}
=\frac{1}{K}
\left[
\frac{1}{|S|}-\delta_{i=j}
+\frac{B_j}{\sqrt{A}}
\cdot\left(\frac{1}{|S|}-\alpha_i\right)
\right]
\]
Note that
\[
\frac{B_j}{K}=\frac{\sum_{j'\in S}z_{j'}-|S|z_j}
{\sum_{j'\in S}(\nu-z_{j'})}
=\frac{\sum_{j'\in S}(z_{j'}-\nu)+|S|(\nu-z_j)}
{\sum_{j'\in S}(\nu-z_{j'})}
=|S|\alpha_j-1.
\]
Then
\[
J_{ij}
=\frac{\partial\alpha_i}{\partial z_j}
=\frac{1}{K}\left(\frac{1}{|S|}-\delta_{i=j}\right)
-\frac{|S|}{\sqrt{A}}
\left(\alpha_i-\frac{1}{|S|}\right)
\left(\alpha_j-\frac{1}{|S|}\right).
\]
% We can do a sanity check by noticing that
% \[
% \sum_i\frac{\partial\alpha_i}{\partial z_j}
% =\frac{\partial\sum_i\alpha_i}{\partial z_j}
% =\frac{\partial 1}{\partial z_j}=0.
% \]
In matrix form,
\[
J=\frac{1}{K}
\left(\frac{\svec\svec^\top}{|S|}-\Diag(\svec)\right)
-\frac{|S|}{\sqrt{A}}
\left(\alphavec\circ\svec-\frac{\svec}{|S|}\right)
\left(\alphavec\circ\svec-\frac{\svec}{|S|}\right)^\top,
\]
where $s_i=\delta_{i\in S}$ and $\circ$ is element-wise multiplication. 
More often, we need to compute its multiplication with a vector $\vvec$
\[
J\vvec=
\frac{\svec}{K}\circ\left(\frac{\svec^\top\vvec}{|S|}
-\vvec\right)
-\frac{|S|}{\sqrt{A}}
\left(\alphavec\circ\svec-\frac{\svec}{|S|}\right)
\left(\alphavec\circ\svec-\frac{\svec}{|S|}\right)^\top
\vvec.
\]
Note that all quantities except $A$ have been computed during the forward pass of calculating \cref{eq:sharpmax}.
$A$ can be computed in $O(|S|)$ time so the overall computation is still $O(|S|)$.

\section{Surrogates}

(1)~Replacing with $\frac{\tau}{2}\|\alphavec\|_2^2$. 
%~$F^*(\alpha)=\frac{\tau}{2}\|\alpha\|_2^2$. 
Then

\begin{equation}
\min_{\alphavec\in\Delta}\quad
U_h(\alphavec)=
-\langle -\gvec_h, \alphavec \rangle + \frac{\tau}{2} \|\alphavec\|_2^2
=\frac{\tau}{2}\left(
\left\|(-\gvec_h/\tau)-\alphavec\right\|_2^2
-\left\|-\gvec_h/\tau\right\|_2^2\right)
\label{eq:L2_problem}
\end{equation}

It is not hard to see that given $h$, the minimum and minimizer of \cref{eq:L2_problem} are 
\begin{equation}
U_h^*=\langle \gvec_h, \alphavec^* \rangle + \frac{\tau}{2}\|\alphavec^*\|_2^2,
\qquad
\alphavec^*=\argmin_{\alphavec\in\Delta} 
\|(-\gvec_h/\tau)-\alphavec\|_2^2
=\sparsemax(-\gvec_h/\tau)
\label{eq:L2_alpha}
\end{equation}
% Plugging in this $\alpha^*$, the optimum is
% U(\alpha^*) = -F(-g/\tau)
% = \min_{\alpha\in\Delta}\frac{1}{2}\|(-g/\tau)-\alpha\|_2^2
% - \frac{1}{2}\|g/\tau\|_2^2
% \qquad
The $\alphavec^*$ is the projection of $-\gvec_h/\tau$ onto the $\Delta$ with the minimum $L_2$ distance, which can be solved in $O(k\log k)$ time using sorting. 
Note that some of the domains may be completely ignored for this $\alphavec^*$ (i.e., $\alpha_i^*=0$ for some $i$).

(2)~Replacing with $-\tau H(\alphavec)$ where $H$ is the Shannon entropy. 
%~$F^*(\alpha)=-\tau H(\alpha)$ where $H$ is the entropy function. 
Then
\begin{equation}
\min_{\alphavec\in\Delta}\quad
U_h(\alphavec) = -\langle -\gvec_h, \alphavec\rangle - \tau H(\alphavec)
\label{eq:softmax_problem}
\end{equation}

\begin{proposition}
Given h, the minimum and minimizer of \cref{eq:softmax_problem} are
\begin{equation}
U^*_h = -\tau\log\sum_i\exp(-g_{h,i}/\tau),
\qquad
\alphavec^*=\softmax(-\gvec_h/\tau)
\label{eq:softmax_alpha}
\end{equation}
\end{proposition}
\begin{proof}
Use the following lemma
\[
D_{F^*}(\pvec_2\|\pvec_1)
= F(\qvec_1) - \langle \qvec_1,\pvec_2\rangle + F^*(\pvec_2).
\]
Set $F^*(\alphavec)=-\tau H(\alphavec)$ and $F(-\gvec_h)=\tau\log\sum_i\exp(-g_{h,i}/\tau)$.
Then we can rewrite $U_h(\alphavec)$ as
\[
U_h(\alphavec)
= \left[F(-\gvec_h)
-\langle -\gvec_h, \alphavec\rangle 
+ F^*(\alphavec)\right]
- F(-\gvec_h)
= D_{F^*}(\alphavec\|\alphavec^*) - F(-\gvec_h),
\]
where $D_{F^*}$ in our case is the (tempered) KL divergence and $\alphavec^*=\nabla F(-\gvec_h)=\softmax(-\gvec_h/\tau)$. 
Given $h$ (or equivalently $\gvec_h$), to minimize $U_h(\alphavec)$, we will pick $\alphavec=\alphavec^*$ so that $D_{F^*}=0$ and the minimum is then $U^*_h=-F(-\gvec_h)$.
\end{proof}
% Based on Bregman divergence minimization~\citep{banerjee2005clustering,norouzi2016reward}, we can solve this analytically:
Here $\tau$ serves as a temperature parameter. 
It is guaranteed to use all domains, whereas the $L_2^2$ approach above may drop some source domains.
